SpooFL: Spoofing Federated Learning

Traditional defenses against Deep Leakage (DL) attacks in Federated Learning (FL) primarily focus on obfuscation, introducing noise, transformations or encryption to degrade an attacker's ability to reconstruct private data. While effective to some extent, these methods often still leak high-level information such as class distributions or feature representations, and are frequently broken by increasingly powerful denoising attacks. We propose a fundamentally different perspective on FL defense: framing it as a spoofing problem.We introduce SpooFL (Figure 1), a spoofing-based defense that deceives attackers into believing they have recovered the true training data, while actually providing convincing but entirely synthetic samples from an unrelated task. Unlike prior synthetic-data defenses that share classes or distributions with the private data and thus still leak semantic information, SpooFL uses a state-of-the-art generative model trained on an external dataset with no class overlap. As a result, attackers are misled into recovering plausible yet completely irrelevant samples, preventing meaningful data leakage while preserving FL training integrity. We implement the first example of such a spoofing defense, and evaluate our method against state-of-the-art DL defenses and demonstrate that it successfully misdirects attackers without compromising model performance significantly.

==> sec/0_abstract.tex <==
\vspace{-15pt}
\begin{abstract}
Traditional defenses against Deep Leakage (DL) attacks in Federated Learning (FL) primarily focus on obfuscation, introducing noise, transformations or encryption to degrade an attacker's ability to reconstruct private data. However, even when successful, these approaches often still allow leakage of high-level information, such as class distributions and feature representations. They are also hard to future-proof, frequently being overcome by increasingly sophisticated denoising attacks. We propose a radically different way of thinking about FL defense; as a spoofing problem. We demonstrate this with a spoofing-based defense called SpooFL (Figure \ref{fig:spoofl}) that aims to trick the attacker into believing they have successfully recovered the real training data while actually providing them with entirely synthetic samples on unrelated tasks. While some existing defenses have explored synthetic data proxies, they are typically drawn from the same classes and data distribution as the private data, meaning that class and feature information can still be leaked. Our approach eliminates this risk by using a state-of-the-art generative models trained on an external dataset with no overlapping classes, ensuring that the attack recovers convincing but completely unrelated samples. This convinces the attacker that an entirely different problem is being solved, preventing meaningful data leakage while preserving FL training integrity. We implement the first example of such a spoofing defense, and evaluate our method against state-of-the-art DL defenses and demonstrate that it successfully misdirects attackers without compromising model performance significantly.
\end{abstract}
\vspace{-15pt}
